A Compositional Framework for Preference-Aware Agents

A formal description of a Cyber-Physical system should include a rigorous specification of the computational and physical components involved, as well as their interaction. Such a description, thus, lends itself to a compositional model where every module in the model specifies the behavior of a (computational or physical) component or the interaction between different components. We propose a framework based on Soft Constraint Automata that facilitates the component-wise description of such systems and includes the tools necessary to compose subsystems in a meaningful way, to yield a description of the entire system. Most importantly, Soft Constraint Automata allow the description and composition of components' preferences as well as environmental constraints in a uniform fashion. We illustrate the utility of our framework using a detailed description of a patrolling robot, while highlighting methods of composition as well as possible techniques to employ them.

==> eptcsdata.tex <==
\providecommand{\firstpage}{21}
\providecommand{\publicationstatus}{Kargahi and Trivedi: Verification and Validation of \\Cyber-Physical Systems 2016 (V2CPS-16)\\
EPTCS 232, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.232.6}{10.4204/EPTCS.232.6}}
\pdfoutput=1

